Tame algebra estimates for product and flag kernels on graded Lie groups

We prove that product kernels and flag kernels on a direct product of graded Lie groups $G_1 \times \cdots \times G_{\nu}$ satisfy so-called \emph{tame algebra estimates}. Tame algebra estimates are central to the study of nonlinear partial differential equations via, for instance, the Nash-Moser inverse function theorem. In addition, the special structure of these estimates generates a new Banach-algebraic proof of an inversion theorem for product kernels and flag kernels.

==> proof_of_tame_estimate_for_pks.tex <==
\begin{proof}

We first separate the summands into three cases associated to $S= \emptyset$, nonempty subsets $S \subsetneq \{1, \ldots, \nu\}$, and $S = \{1, \ldots, \nu\}$. That is, we have
\begin{equation}\label{eq pk KL step 1}
    \begin{split}
        \norm{K*L}{(k_1, k_2)}\leq &  \norm{\Op(K)}{\mB(L^2(\R^q))} \norm{\Op(L)}{\mB(L^2(\R^q))}\\
    &+\sup_{\substack{\norm{f}{L^2(\R^q)}  =1;\\
        \norm{g}{L^2(\R^q)} =1 }} \sup_{w \in \R^{q}} \sup_{\substack{z\in \R^q; \\ |w_{\mu} z_{\mu}^{-1}|_{\mu} \geq 10; \\ \mu =1, \ldots, \nu }}
        \sum_{\substack{S \subsetneq \{1, \ldots, \nu\}; \\ S \neq \emptyset }} \sum_{|\ap^S| \leq \vk^S} \lf \Big\la \bigotimes_{\mu \in S} \phi_{\mu} f, X^{\ap^S}( K*L)* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
        &\prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }\\
        &+\sup_{\substack{\norm{f}{L^2(\R^q)}  =1;\\
        \norm{g}{L^2(\R^q)} =1 }} \sup_{w \in \R^{q}} \sup_{\substack{z\in \R^q; \\ |w_{\mu} z_{\mu}^{-1}|_{\mu} \geq 10; \\ \mu =1, \ldots, \nu }}
         \sum_{|\ap| \leq \vk} \lf \Big\la \bigotimes_{\mu =1}^{\nu} \phi_{\mu} f, X^{\ap}( K*L)* \bigotimes_{\mu =1}^{\nu} \g_{\mu} g \Big\ra \rf \\
        &\prod_{\mu=1}^{\nu} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }
    \end{split}
\end{equation}
It thus remains to bound the second and third terms in \eqref{eq pk KL step 1}. 


\subsubsection{2nd term} \ 

We start by estimating the second term in \eqref{eq pk KL step 1}, associated to all nonempty subsets $S \subsetneq \{1, \ldots, \nu\}$,
\begin{equation}\label{eq pk KL term 2}
    \begin{split}
        &\sup_{\substack{\norm{f}{L^2(\R^q)}  =1;\\
        \norm{g}{L^2(\R^q)} =1 }} \sup_{w \in \R^{q}} \sup_{\substack{z\in \R^q; \\ |w_{\mu} z_{\mu}^{-1}|_{\mu} \geq 10; \\ \mu =1, \ldots, \nu }}
        \sum_{\substack{S \subsetneq \{1, \ldots, \nu\}; \\ S \neq \emptyset }} \sum_{|\ap^S| \leq \vk^S} \lf \Bigg\la \bigotimes_{\mu \in S} \phi_{\mu} f, X^{\ap^S}( K*L)* \bigotimes_{\mu \in S} \g_{\mu} g \Bigg\ra \rf \\
        &\prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }
    \end{split}
\end{equation}

Let $\phi_{\mu} \prec \vp_{\mu}$ s.t. $\dist(\supp \phi_{\mu}, \supp (1-\vp_{\mu} )) \geq 10$. By the triangle inequality and bilinearity of convolution, 
\begin{equation}\label{eq pk kl intro phi}
    \begin{split}
        & \sum_{|\ap^S| \leq \vk^S} \lf \Bigg\la \bigotimes_{\mu \in S} \phi_{\mu} f, X^{\ap^S}( K*L)* \bigotimes_{\mu \in S} \g_{\mu} g \Bigg\ra \rf \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }\\
        & \leq \sum_{|\ap^S| \leq \vk^S} \lf \Bigg\la \bigotimes_{\mu \in S} \phi_{\mu} f, X^{\ap^S}\Big( K* \bigotimes_{\mu \in S} \vp_{\mu} L\Big)* \bigotimes_{\mu \in S} \g_{\mu} g \Bigg\ra \rf \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \\
        & + \sum_{|\ap^S| \leq \vk^S} \sum_{S' \subsetneq S} \lf \Big\la \bigotimes_{\mu \in S} \phi_{\mu} f, X^{\ap^S}\Big( K* \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
        \bigotimes_{\mu_2 \in S\backslash S'} (1-\vp_{\mu_2}) L\Big)* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \\
        &+ \sum_{|\ap^S| \leq \vk^S} \lf \Big\la \bigotimes_{\mu \in S} \phi_{\mu} f, X^{\ap^S}\Big( K* \bigotimes_{\mu \in S} (1-\vp_{\mu}) L\Big)* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } 
    \end{split}
\end{equation}

In order to apply the differential operator $X^{\ap_{\mu}}$ to the distribution which is localized away from its singularity in $\R^{q_{\mu}}$, we write the \textit{left-invariant} vector field as linear combinations of \textit{right-invariant} vector field:
\begin{align*}
    X^{\ap_{\mu}} = \sum_{\substack{|\beta_{\mu}| \leq |\ap_{\mu}|; \\ \deg \beta_{\mu} \geq \deg \ap_{\mu}}} p_{\ap_{\mu}, \beta_{\mu}} Y^{\beta_{\mu}}
\end{align*}
where $p_{\ap, \beta}$ are homogeneous polynomials\footnote{See Proposition 1.29 p.26 in \cite{FS82} for a proof of this identity.} of homogeneous degree $\deg \beta_{\mu} - \deg \ap_{\mu}$. In addition, given a left-invariant vector fields $X$, we have $X(f*g) = f* (Xg)$ and similarly given a right-invariant vector field $Y$, we have $Y(f*g) = (Yf) *g$. As such, \eqref{eq pk kl intro phi} is
\begin{equation}\label{eq pk kl phi and Y}
    \begin{split}
        &\lesssim \sum_{|\ap^S| \leq \vk^S} \lf \Bigg\la \bigotimes_{\mu \in S} \phi_{\mu} f, \Big( K* \bigotimes_{\mu \in S} \wt{\vp}_{\mu} X^{\ap^S} L\Big)* \bigotimes_{\mu \in S} \g_{\mu} g \Bigg\ra \rf \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \\
        & + \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{S' \subsetneq S} \lf \Big\la \bigotimes_{\mu \in S} \phi_{\mu} f, p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} Y^{\beta^{S \backslash S'}} X^{\beta^{S'}}\Big( K* \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
        \bigotimes_{\mu_2 \in S\backslash S'} (1-\vp_{\mu_2}) L\Big)* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
        &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \\
        &+ \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \lf \Big\la \bigotimes_{\mu \in S} \phi_{\mu} f, p_{(\ap^S, \beta^S)} Y^{\beta^S} \Big( K* \bigotimes_{\mu \in S} (1-\vp_{\mu}) L\Big)* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } 
    \end{split}
\end{equation}
where $p_{\ap^S, \beta^S}$ are homogeneous polynomials. 

Let $\g_{\mu}^{j, n} \in C^{\infty}_c(\R^{q_{\mu}})$ be chosen so that $\supp \g_{\mu}^{j, n} \subseteq B^{q_{\mu}} (z_{\mu}^{j, n}, 1)$, $0 \leq \g_{\mu}^{j, n} \leq 1$ and $|w_{\mu}^{-1}z_{\mu}^{j, n}|_{\mu} \sim n$\footnote{Recall $w_{\mu}$ is the center of the ball of radius $1$ containing $\supp \phi_{\mu}$. That is, $\supp \phi_{\mu} \subseteq B^{q_{\mu}} (w_{\mu}, 1)$}. By the doubling condition of the metric on $\R^{q_{\mu}}$, each annulus in $\R^{q_{\mu}}$, centered at $w_{\mu}$, of outer radius $n$ and inner radius $n-2$ contains at most a constant multiple of $n^{Q_{\mu} -1}$ unit balls\footnote{For each such annulus, there are $n^{Q_{\mu}} - (n-2)^{Q_{\mu}}\sim n^{Q_{\mu}-1}$ unit balls in the annulus.}. 

We thus obtain a decomposition of the function $(1-\vp_{\mu})$:
\begin{equation}\label{eq decomp vp}
    1-\vp_{\mu} = \sum_{n \geq 5} \sum_{j =1 }^{n^{Q_{\mu} -1}} \g_{\mu}^{j, n}. 
\end{equation}
where for each $j, n$, we have $\supp \g_{\mu}^{j, n} \subseteq B^{q_{\mu}} (z_{\mu}^{j, n}, 1)$. 

By substituting the decomposition in \eqref{eq decomp vp} into \eqref{eq pk kl phi and Y} and by the triangle inequality, \eqref{eq pk kl phi and Y} is
\begin{align*}
    &\lesssim \sum_{|\ap^S| \leq \vk^S} \lf \Bigg\la \bigotimes_{\mu \in S} \phi_{\mu} f, \Big( K* \bigotimes_{\mu \in S} \wt{\vp}_{\mu} X^{\ap^S} L\Big)* \bigotimes_{\mu \in S} \g_{\mu} g \Bigg\ra \rf \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \\
    & + \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}}  \sum_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S'; \\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \\
    &\lf \Big\la \bigotimes_{\mu \in S} \phi_{\mu} f, p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})}   \Big( (Y^{\beta^{S \backslash S'}} K)* X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
    \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} L\Big)* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
    &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \\
    &+ \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{\substack{n_{\mu} \geq 5; \\ \mu \in S}} \sum_{j_{\mu} =1 }^{n_{\mu}^{Q_{\mu} -1}} \lf \Big\la \bigotimes_{\mu \in S} \phi_{\mu} f, p_{(\ap^S, \beta^S)}  \Big( ( Y^{\beta^S} K)* \bigotimes_{\mu \in S}  \g_{\mu}^{j_{\mu}, n_{\mu}} L\Big)* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
    &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } 
\end{align*}
By taking adjoints, we rewrite the equation above as
\begin{equation}\label{eq after separating K and L}
\begin{split}
    &\lesssim \sum_{|\ap^S| \leq \vk^S} \lf \Bigg\la \wt{K}* \bigotimes_{\mu \in S} \phi_{\mu} f,  \bigotimes_{\mu \in S} \wt{\vp}_{\mu} X^{\ap^S} L* \bigotimes_{\mu \in S} \g_{\mu} g \Bigg\ra \rf \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \\
    & + \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}}  \sum_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \\
    &\lf \Big\la \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} * \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } \bigotimes_{\mu \in S} \phi_{\mu} f,    X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
     L* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
    &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \\
    &+ \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{\substack{n_{\mu} \geq 5; \\ \mu \in S}} \sum_{j_{\mu} =1 }^{n_{\mu}^{Q_{\mu} -1}} \lf \Big\la \bigotimes_{\mu \in S}  \g_{\mu}^{j_{\mu}, n_{\mu}} ( Y^{\beta^S} K)^{\sim} * \overline{p_{\ap^S, \beta^S}}\bigotimes_{\mu \in S} \phi_{\mu} f,    L * \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
    & \hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } 
    \end{split}
\end{equation}
where $\wt{K}$ is the kernel of the adjoint operator $\Op(K)^*$. Formally, we have $\wt{K}(t) = \overline{K}(t^{-1})$. 


We bound the first term in \eqref{eq after separating K and L} with the following lemma.
\begin{lemma}\label{lemma pk kl aps}
We have
    \begin{equation}
        \begin{split}
            \sum_{|\ap^S| \leq \vk^S} \lf \Bigg\la \wt{K}* \bigotimes_{\mu \in S} \phi_{\mu} f,  \bigotimes_{\mu \in S} \wt{\vp}_{\mu} X^{\ap^S} L* \bigotimes_{\mu \in S} \g_{\mu} g \Bigg\ra \rf \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } & \lesssim \norm{\Op(K)}{\mB(L^2(\R^q))} \norm{L}{\vk^S_0}
        \end{split}
    \end{equation}
\end{lemma}


\begin{proof}[Proof of Lemma \ref{lemma pk kl aps}]
By Cauchy-Schwartz, we can separate the two product kernels
    \begin{align*}
        &\sum_{|\ap^S| \leq \vk^S} \lf \Bigg\la \wt{K}* \bigotimes_{\mu \in S} \phi_{\mu} f,  \bigotimes_{\mu \in S} \wt{\vp}_{\mu} X^{\ap^S} L* \bigotimes_{\mu \in S} \g_{\mu} g \Bigg\ra \rf \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }\\
        & \lesssim \norm{\Op(\wt{K})}{\mB(L^2(\R^q))} \sum_{|\ap^S| \leq \vk^S} \norm{\bigotimes_{\mu \in S} \wt{\vp}_{\mu} X^{\ap^S} L* \bigotimes_{\mu \in S} \g_{\mu} g}{L^2(\R^q)} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }
    \end{align*}
    where the $L^2$ operator norms of $\Op(K)$ and $\Op(\wt{K}) = \Op(K)^*$ are the same. In addition, we recognize the $\vk^S_0$ norm of the distribution $L$. That is, we have
    \begin{align*}
        &\lesssim \norm{\Op(\wt{K})}{\mB(L^2(\R^q))} \norm{L}{\vk^S_0}.
    \end{align*}
    Thus proving the lemma. 
\end{proof}

We bound the second term in \eqref{eq after separating K and L} in the next lemma.

\begin{lemma}\label{lemma pk kl S'}
    \begin{equation}
        \begin{split}
            &\sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}}  \sum_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \\
            &\lf \Big\la \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} * \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } \bigotimes_{\mu \in S} \phi_{\mu} f,    X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
     L* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
            &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }\\
            & \lesssim ?
        \end{split}
    \end{equation}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lemma pk kl S'}]
We thus separate the sum into two cases:
when $|w_{\mu}z_{\mu}^{-1}| \leq n_{\mu}$ and $|w_{\mu}z_{\mu}^{-1}| \geq n_{\mu}$.
\begin{align*}
        &\sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}}  \sum_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \\
        &\lf \Big\la \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} * \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } \bigotimes_{\mu \in S} \phi_{\mu} f,    X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
     L* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
        &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }\\
        & \lesssim \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}}  \Big( \sum_{\substack{5 \leq n_{\mu_2} \leq |w_{\mu}z_{\mu}^{-1}|; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \\
        &\lf \Big\la \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} * \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } \bigotimes_{\mu \in S} \phi_{\mu} f,    X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
     L* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
        &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }\\
        & + \sum_{\substack{5 \leq |w_{\mu}z_{\mu}^{-1}| \leq n_{\mu_2}  ; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \\
        &\lf \Big\la \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} * \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } \bigotimes_{\mu \in S} \phi_{\mu} f,    X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
     L* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
        &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \Big)
    \end{align*}

    For the second summand, by applying Cauchy-Schwartz followed by Hölder's inequality, 
    \begin{align*}
        &\sum_{\substack{5 \leq |w_{\mu}z_{\mu}^{-1}| \leq n_{\mu_2}  ; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \lf \Big\la \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} * \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } \bigotimes_{\mu \in S} \phi_{\mu} f,    X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
     L* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
        &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }\\
        & \leq \sum_{\substack{5 \leq |w_{\mu}z_{\mu}^{-1}| \leq n_{\mu_2}  ; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sup_{j_{\mu_2}} \prod_{\mu_2 \in S \backslash S'} n_{\mu_2}^{-Q_{\mu_2} - \deg \ap_{\mu_2}} n_{\mu_2}^{Q_{\mu_2} -1} \\
        &\lf \Big\la \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} * \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } \bigotimes_{\mu \in S} \phi_{\mu} f,    X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
     L* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
        &\hspace{3in} \prod_{\mu_2 \in S \backslash S'} n_{\mu_2}^{Q_{\mu_2} + \deg \ap_{\mu_2}} \prod_{\mu_1 \in S'} (1+ |w_{\mu_1} z_{\mu_1}^{-1}|_{\mu_1})^{Q_{\mu_1} + \deg \ap_{\mu_1} }
    \end{align*}

    \AS{deal with the polynomial}

    \vspace{.5in}

    For the first summand, we separate further into two subcases: $5 \leq n_{\mu_2} \leq |w_{\mu}z_{\mu}^{-1}|/2$ and $|w_{\mu}z_{\mu}^{-1}|/2 \leq n_{\mu_2} \leq |w_{\mu}z_{\mu}^{-1}|$. The first sub-case corresponds to test functions $\g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}}$ with centers at a distance at least $|w_{\mu}z_{\mu}^{-1}|/2$ away from $\g_{\mu}$ and at most $|w_{\mu}z_{\mu}^{-1}|/2$ away from $\phi_{\mu}$. As such, we will place the differential operators on $L$. The second sub-case corresponds to test functions $\g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}}$ with centers at a distance at least $|w_{\mu}z_{\mu}^{-1}|/2$ and at most $|w_{\mu}z_{\mu}^{-1}|$ from $\phi_{\mu}$. We thus place the differential operators on $K$. 
    \begin{align*}
        &\sum_{\substack{5 \leq n_{\mu_2} \leq |w_{\mu}z_{\mu}^{-1}|; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \lf \Big\la \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} * \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } \bigotimes_{\mu \in S} \phi_{\mu} f,    X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
     L* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
        &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }\\
        &\leq \sum_{\substack{5 \leq n_{\mu_2} \leq |w_{\mu}z_{\mu}^{-1}|/2; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \lf \Big\la \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} * \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } \bigotimes_{\mu \in S} \phi_{\mu} f,    X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
     L* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
        &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }\\
        &+\sum_{\substack{|w_{\mu}z_{\mu}^{-1}|/2 \leq n_{\mu_2} \leq |w_{\mu}z_{\mu}^{-1}|; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \lf \Big\la \bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} * \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } \bigotimes_{\mu \in S} \phi_{\mu} f,    X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} 
     L* \bigotimes_{\mu \in S} \g_{\mu} g \Big\ra \rf \\
        &\hspace{4in} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }
    \end{align*}
\end{proof}


\vspace{1in}


By Cauchy-Schwartz, we can finally separate the two product kernels $K$ and $L$,
\begin{align*}
    &\lesssim \norm{\Op(\wt{K})}{\mB(L^2(\R^q))} \sum_{|\ap^S| \leq \vk^S} \norm{\bigotimes_{\mu \in S} \wt{\vp}_{\mu} X^{\ap^S} L* \bigotimes_{\mu \in S} \g_{\mu} g }{L^2(\R^q)} \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \\
    & + \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}}  \sum_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \norm{\bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} *  \bigotimes_{\mu \in S} \phi_{\mu} \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } f}{L^(\R^q)} \\
    & \prod_{\mu_2 \in S \backslash S'} (1+ |w_{\mu_2} z_{\mu_2}^{-1}|_{\mu_2})^{Q_{\mu_2} + \deg \ap_{\mu_2} } \norm{X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} L* \bigotimes_{\mu \in S} \g_{\mu} g}{L^2(\R^q)}  \prod_{\mu_1 \in S'} (1+ |w_{\mu_1} z_{\mu_1}^{-1}|_{\mu_1})^{Q_{\mu_1} + \deg \ap_{\mu_1} } \\
    &+ \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{\substack{n_{\mu} \geq 5; \\ \mu \in S}} \sum_{j_{\mu} =1 }^{n_{\mu}^{Q_{\mu} -1}} 
    \norm{\bigotimes_{\mu \in S}  \g_{\mu}^{j_{\mu}, n_{\mu}} ( Y^{\beta^S} K)^{\sim} * \bigotimes_{\mu \in S} \phi_{\mu} \overline{p_{\ap^S, \beta^S}} f}{L^2(\R^q)}\\
    & \hspace{1in}  \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \norm{\Op(L)}{\mB(L^2(\R^q))}
\end{align*}
Observe that $\deg \ap_{\mu_1} \leq \deg \beta_{\mu_1}$.  \AS{$\wt{\vp}_{\mu}$ and $\phi_{\mu}$}
\begin{align*}
    &\lesssim \norm{\Op(K)}{\mB(L^2(\R^q))} \norm{L}{\vk^S_0} \\
    & + \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}}  \sum_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S';\\ S' \subsetneq S }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \norm{\bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} *  \bigotimes_{\mu \in S} \phi_{\mu} \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } f}{L^(\R^q)} \\
    & \prod_{\mu_2 \in S \backslash S'} (1+ |w_{\mu_2} z_{\mu_2}^{-1}|_{\mu_2})^{Q_{\mu_2} + \deg \ap_{\mu_2} } \norm{X^{\beta^{S'}} \bigotimes_{\mu_1 \in S'} \vp_{\mu_1} L* \bigotimes_{\mu \in S} \g_{\mu} g}{L^2(\R^q)}  \prod_{\mu_1 \in S'} (1+ |w_{\mu_1} z_{\mu_1}^{-1}|_{\mu_1})^{Q_{\mu_1} + \deg \beta_{\mu_1} } \\
    &+ \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{\substack{n_{\mu} \geq 5; \\ \mu \in S}} \sum_{j_{\mu} =1 }^{n_{\mu}^{Q_{\mu} -1}} 
    \norm{\bigotimes_{\mu \in S}  \g_{\mu}^{j_{\mu}, n_{\mu}} ( Y^{\beta^S} K)^{\sim} * \bigotimes_{\mu \in S} \phi_{\mu} \overline{p_{\ap^S, \beta^S}} f}{L^2(\R^q)}\\
    & \hspace{1in}  \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \norm{\Op(L)}{\mB(L^2(\R^q))}
\end{align*}
We recognize another seminorm.
\begin{align*}
    &\lesssim \norm{\Op(K)}{\mB(L^2(\R^q))} \norm{L}{\vk^S_0} \\
    & + \sum_{S' \subsetneq S} \sum_{|\ap^{S \backslash S'}| \leq \vk^{S \backslash S'}} \sum_{\substack{|\beta^{S \backslash S'}| \leq |\ap^{S \backslash S'}|; \\ \deg \beta^{S \backslash S'} \geq \deg \ap^{S \backslash S'}}}  \sum_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S' }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \norm{\bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} *  \bigotimes_{\mu \in S} \phi_{\mu} \overline{ p_{(\ap^{S\backslash S'}, \beta^{S\backslash S'})} } f}{L^(\R^q)} \\
    & \prod_{\mu_2 \in S \backslash S'} (1+ |w_{\mu_2} z_{\mu_2}^{-1}|_{\mu_2})^{Q_{\mu_2} + \deg \ap_{\mu_2} } \norm{L}{\vk^{S'}_0}\\
    &+ \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{\substack{n_{\mu} \geq 5; \\ \mu \in S}} \sum_{j_{\mu} =1 }^{n_{\mu}^{Q_{\mu} -1}} 
    \norm{\bigotimes_{\mu \in S}  \g_{\mu}^{j_{\mu}, n_{\mu}} ( Y^{\beta^S} K)^{\sim} * \bigotimes_{\mu \in S} \phi_{\mu} \overline{p_{\ap^S, \beta^S}} f}{L^2(\R^q)}\\
    & \hspace{1in}  \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \norm{\Op(L)}{\mB(L^2(\R^q))}
\end{align*}


\AS{Given $w_{\mu_2}$, sup over $z_{\mu_2}$. So we need to have $|w_{\mu_2}|_{\mu_2}\geq |w_{\mu_2}z_{\mu_2}^{-1}|_{\mu_2}$. In the other case, I would have something that would not be a supremum over the $z$'s given a $w$. } \AS{instead, use translation-invariance}

\begin{align*}
    &\lesssim \norm{\Op(K)}{\mB(L^2(\R^q))} \norm{L}{\vk^S_0} \\
    & + \sum_{S' \subsetneq S} \sum_{|\ap^{S \backslash S'}| \leq \vk^{S \backslash S'}} \sum_{\substack{|\beta^{S \backslash S'}| \leq |\ap^{S \backslash S'}|; \\ \deg \beta^{S \backslash S'} \geq \deg \ap^{S \backslash S'}}}  \sum_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S' }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \norm{\bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} *  \bigotimes_{\mu \in S} \phi_{\mu} }{\mB(L^(\R^q))} \\
    & \prod_{\mu_2 \in S \backslash S'} |w_{\mu_2}|_{\mu_2}^{\deg \beta_{\mu_2} - \deg \ap_{\mu_2}} (1+ |w_{\mu_2} z_{\mu_2}^{-1}|_{\mu_2})^{Q_{\mu_2} + \deg \ap_{\mu_2} } \norm{L}{\vk^{S'}_0}\\
    &+ \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{\substack{n_{\mu} \geq 5; \\ \mu \in S}} \sum_{j_{\mu} =1 }^{n_{\mu}^{Q_{\mu} -1}} 
    \norm{\bigotimes_{\mu \in S}  \g_{\mu}^{j_{\mu}, n_{\mu}} ( Y^{\beta^S} K)^{\sim} * \bigotimes_{\mu \in S} \phi_{\mu} \overline{p_{\ap^S, \beta^S}} f}{L^2(\R^q)}\\
    & \hspace{1in}  \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \norm{\Op(L)}{\mB(L^2(\R^q))}
\end{align*}

\begin{align*}
    &\lesssim \norm{\Op(K)}{\mB(L^2(\R^q))} \norm{L}{\vk^S_0} \\
    & + \sum_{S' \subsetneq S} \sum_{|\ap^{S \backslash S'}| \leq \vk^{S \backslash S'}} \sum_{\substack{|\beta^{S \backslash S'}| \leq |\ap^{S \backslash S'}|; \\ \deg \beta^{S \backslash S'} \geq \deg \ap^{S \backslash S'}}}  \sum_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S' }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \norm{\bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} *  \bigotimes_{\mu \in S} \phi_{\mu} }{\mB(L^(\R^q))} \\
    & \prod_{\mu_2 \in S \backslash S'}  (1+ |w_{\mu_2} z_{\mu_2}^{-1}|_{\mu_2})^{Q_{\mu_2} + \deg \beta_{\mu_2} } \norm{L}{\vk^{S'}_0}\\
    &+ \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{\substack{n_{\mu} \geq 5; \\ \mu \in S}} \sum_{j_{\mu} =1 }^{n_{\mu}^{Q_{\mu} -1}} 
    \norm{\bigotimes_{\mu \in S}  \g_{\mu}^{j_{\mu}, n_{\mu}} ( Y^{\beta^S} K)^{\sim} * \bigotimes_{\mu \in S} \phi_{\mu} \overline{p_{\ap^S, \beta^S}} f}{L^2(\R^q)}\\
    & \hspace{1in}  \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \norm{\Op(L)}{\mB(L^2(\R^q))}
\end{align*}


Introducing $n$'s and \AS{recalling what we're supping over}


\begin{align*}
    &\leq \norm{\Op(K)}{\mB(L^2(\R^q))} \norm{L}{\vk^S_0} \\
    & + \sup_{w \in \R^{q}} \sup_{\substack{z\in \R^q; \\ |w_{\mu} z_{\mu}^{-1}|_{\mu} \geq 10; \\ \mu =1, \ldots, \nu }} \sum_{S' \subsetneq S} \sum_{|\ap^{S \backslash S'}| \leq \vk^{S \backslash S'}} \sum_{\substack{|\beta^{S \backslash S'}| \leq |\ap^{S \backslash S'}|; \\ \deg \beta^{S \backslash S'} \geq \deg \ap^{S \backslash S'}}}  \sum_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S' }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \norm{\bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} *  \bigotimes_{\mu \in S} \phi_{\mu} }{\mB(L^2(\R^q))} \\
    & \prod_{\mu_2 \in S \backslash S'}  (1+ |w_{\mu_2} z_{\mu_2}^{-1}|_{\mu_2})^{Q_{\mu_2} + \deg \beta_{\mu_2} } n_{\mu_2}^{Q_{\mu_2} + \deg \beta_{\mu_2}} n_{\mu_2}^{-Q_{\mu_2} - \deg \beta_{\mu_2}} \norm{L}{\vk^{S'}_0}\\
    &+ \sup_{w \in \R^{q}} \sup_{\substack{z\in \R^q; \\ |w_{\mu} z_{\mu}^{-1}|_{\mu} \geq 10; \\ \mu =1, \ldots, \nu }} \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{\substack{n_{\mu} \geq 5; \\ \mu \in S}} \sum_{j_{\mu} =1 }^{n_{\mu}^{Q_{\mu} -1}} 
    \norm{\bigotimes_{\mu \in S}  \g_{\mu}^{j_{\mu}, n_{\mu}} ( Y^{\beta^S} K)^{\sim} * \bigotimes_{\mu \in S} \phi_{\mu} \overline{p_{\ap^S, \beta^S}} f}{L^2(\R^q)}\\
    & \hspace{1in}  \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \norm{\Op(L)}{\mB(L^2(\R^q))}
\end{align*}

Break up the $n_{\mu_2}$ sum into two cases:
\begin{enumerate}
    \item $n_{\mu_2} \leq |w_{\mu}z_{\mu}|$ and 

    \item $n_{\mu_2} \geq |w_{\mu}z_{\mu}|$
\end{enumerate}


\begin{align*}
    &\lesssim \norm{\Op(K)}{\mB(L^2(\R^q))} \norm{L}{\vk^S_0} \\
    & + \sup_{w \in \R^{q}} \sup_{\substack{z\in \R^q; \\ |w_{\mu} z_{\mu}^{-1}|_{\mu} \geq 10; \\ \mu =1, \ldots, \nu }} \sum_{S' \subsetneq S} \sum_{|\ap^{S \backslash S'}| \leq \vk^{S \backslash S'}} \sum_{\substack{|\beta^{S \backslash S'}| \leq |\ap^{S \backslash S'}|; \\ \deg \beta^{S \backslash S'} \geq \deg \ap^{S \backslash S'}}}  \\
    &\Big( \sum_{\substack{5 \leq n_{\mu_2} \leq |w_{\mu}z_{\mu_2}^{-1}|; \\ \mu_2 \in S \backslash S' }} \sum_{j_{\mu_2} =1 }^{n_{\mu_2}^{Q_{\mu} -1}} \norm{\bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} *  \bigotimes_{\mu \in S} \phi_{\mu} }{\mB(L^2(\R^q))} \\
    & \prod_{\mu_2 \in S \backslash S'}  (1+ |w_{\mu_2} z_{\mu_2}^{-1}|_{\mu_2})^{Q_{\mu_2} + \deg \beta_{\mu_2} } n_{\mu_2}^{Q_{\mu_2} + \deg \beta_{\mu_2}} n_{\mu_2}^{-Q_{\mu_2} - \deg \beta_{\mu_2}} \norm{L}{\vk^{S'}_0}\\
    & + \sum_{\substack{n_{\mu_2} \geq |w_{\mu}z_{\mu_2}^{-1}|; \\ \mu_2 \in S \backslash S' }} \sup_{j_{\mu_2}} n_{\mu_2}^{Q_{\mu} -1} n_{\mu_2}^{-Q_{\mu_2} - \deg \beta_{\mu_2}}\norm{\bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} *  \bigotimes_{\mu \in S} \phi_{\mu} }{\mB(L^2(\R^q))} \\
    & \prod_{\mu_2 \in S \backslash S'}   n_{\mu_2}^{Q_{\mu_2} + \deg \beta_{\mu_2}}  \norm{L}{\vk^{S'}_0}\Big) \\
    &+ \sup_{w \in \R^{q}} \sup_{\substack{z\in \R^q; \\ |w_{\mu} z_{\mu}^{-1}|_{\mu} \geq 10; \\ \mu =1, \ldots, \nu }} \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{\substack{n_{\mu} \geq 5; \\ \mu \in S}} \sum_{j_{\mu} =1 }^{n_{\mu}^{Q_{\mu} -1}} 
    \norm{\bigotimes_{\mu \in S}  \g_{\mu}^{j_{\mu}, n_{\mu}} ( Y^{\beta^S} K)^{\sim} * \bigotimes_{\mu \in S} \phi_{\mu} \overline{p_{\ap^S, \beta^S}} f}{L^2(\R^q)}\\
    & \hspace{1in}  \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \norm{\Op(L)}{\mB(L^2(\R^q))}
\end{align*}


\vspace{1in}

By Hölder's inequality applied to the sums in $n_{\mu_2}\in \N$, we have
\begin{align*}
    &\leq \norm{\Op(K)}{\mB(L^2(\R^q))} \norm{L}{\vk^S_0} \\
    & + \sup_{w \in \R^{q}} \sup_{\substack{z\in \R^q; \\ |w_{\mu} z_{\mu}^{-1}|_{\mu} \geq 10; \\ \mu =1, \ldots, \nu }} \sum_{S' \subsetneq S} \sum_{|\ap^{S \backslash S'}| \leq \vk^{S \backslash S'}} \sum_{\substack{|\beta^{S \backslash S'}| \leq |\ap^{S \backslash S'}|; \\ \deg \beta^{S \backslash S'} \geq \deg \ap^{S \backslash S'}}}  \\
    & \sup_{\substack{n_{\mu_2} \geq 5; \\ \mu_2 \in S \backslash S' }} \sup_{\substack{j_{\mu_2}; \\ 1 \leq j_{\mu_2} \leq n_{\mu_2}^{Q_{\mu_2} -1}}} \norm{\bigotimes_{\mu_2 \in S\backslash S'}  \g_{\mu_2}^{j_{\mu_2}, n_{\mu_2}} (Y^{\beta^{S \backslash S'}} K)^{\sim} *  \bigotimes_{\mu \in S} \phi_{\mu} }{\mB(L^2(\R^q))} \\
    & \prod_{\mu_2 \in S \backslash S'} (1+ |w_{\mu_2} z_{\mu_2}^{-1}|_{\mu_2})^{Q_{\mu_2} + \deg \beta_{\mu_2} }   n_{\mu_2}^{Q_{\mu_2} + \deg \beta_{\mu_2}}  \norm{L}{\vk^{S'}_0}\\
    &+ \sup_{w \in \R^{q}} \sup_{\substack{z\in \R^q; \\ |w_{\mu} z_{\mu}^{-1}|_{\mu} \geq 10; \\ \mu =1, \ldots, \nu }} \sum_{|\ap^S| \leq \vk^S} \sum_{\substack{|\beta^S| \leq |\ap^S|; \\ \deg \beta^S \geq \deg \ap^S}} \sum_{\substack{n_{\mu} \geq 5; \\ \mu \in S}} \sum_{j_{\mu} =1 }^{n_{\mu}^{Q_{\mu} -1}} 
    \norm{\bigotimes_{\mu \in S}  \g_{\mu}^{j_{\mu}, n_{\mu}} ( Y^{\beta^S} K)^{\sim} * \bigotimes_{\mu \in S} \phi_{\mu} \overline{p_{\ap^S, \beta^S}} f}{L^2(\R^q)}\\
    & \hspace{1in}  \prod_{\mu \in S} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} } \norm{\Op(L)}{\mB(L^2(\R^q))}
\end{align*}
where $\deg \beta_{\mu_2} >0 $.

\vspace{2in}

Recall, $\g_{\mu}^{j_{\mu}, n_{\mu}} \subseteq B^{q_{\mu}}(z_{\mu}^{j_{\mu}, n_{\mu}}, 1 )$, where $|z_{\mu}^{j_{\mu}, n_{\mu}} w_{\mu}^{-1}|_{\mu} \sim n_{\mu}$. 






\vspace{1in}


\AS{before looking at homogeneous polynomials, this is where I was}


where $\deg \ap_1 >0$. By duality, we thus obtain the desired estimate:
\begin{equation}
    \begin{split}
        & \lesssim \sum_{\substack{S \subsetneq \{1, \ldots, \nu \}; \\ S \neq \emptyset }} \norm{\Op(K)}{\mB(L^2)}  \norm{L}{\vk^S_0} + \norm{K}{\vk^S_0} \norm{\Op(L)}{\mB(L^2)}\\
        &+ \sum_{S' \subsetneq S} \norm{K}{\vk^{S \backslash S'}_0} \norm{L}{\vk^{S'}_0}
    \end{split}
\end{equation}

\subsubsection{third term} \ 

Finally, to estimate the third term in \eqref{eq pk KL step 1}, 
\begin{equation}
    \begin{split}
        &\sup_{\substack{\norm{f}{L^2(\R^q)}  =1;\\
        \norm{g}{L^2(\R^q)} =1 }} \sup_{w \in \R^{q}} \sup_{\substack{z\in \R^q; \\ |w_{\mu} z_{\mu}^{-1}|_{\mu} \geq 10; \\ \mu =1, \ldots, \nu }}
         \sum_{|\ap| \leq \vk} \lf \Big\la \bigotimes_{\mu =1}^{\nu} \phi_{\mu} f, X^{\ap}( K*L)* \bigotimes_{\mu =1}^{\nu} \g_{\mu} g \Big\ra \rf \\
        &\prod_{\mu=1}^{\nu} (1+ |w_{\mu} z_{\mu}^{-1}|_{\mu})^{Q_{\mu} + \deg \ap_{\mu} }
    \end{split}
\end{equation}

\end{proof}


